Fine-Tuning or Fine-Failing? Debunking Performance Myths in Large Language Models

Large Language Models (LLMs) have the unique capability to understand and generate human-like text from input queries. When fine-tuned, these models show enhanced performance on domain-specific queries. OpenAI highlights the process of fine-tuning, stating: "To fine-tune a model, you are required to provide at least 10 examples. We typically see clear improvements from fine-tuning on 50 to 100 training examples, but the right number varies greatly based on the exact use case." This study extends this concept to the integration of LLMs within Retrieval-Augmented Generation (RAG) pipelines, which aim to improve accuracy and relevance by leveraging external corpus data for information retrieval. However, RAG's promise of delivering optimal responses often falls short in complex query scenarios. This study aims to specifically examine the effects of fine-tuning LLMs on their ability to extract and integrate contextual data to enhance the performance of RAG systems across multiple domains. We evaluate the impact of fine-tuning on the LLMs' capacity for data extraction and contextual understanding by comparing the accuracy and completeness of fine-tuned models against baseline performances across datasets from multiple domains. Our findings indicate that fine-tuning resulted in a decline in performance compared to the baseline models, contrary to the improvements observed in standalone LLM applications as suggested by OpenAI. This study highlights the need for vigorous investigation and validation of fine-tuned models for domain-specific tasks.

==> notes.tex <==
One significant use case for LLMs is assisting organisational employees in answering queries about information. By leveraging LLMs, employees can quickly access relevant information without extensive manual searches, thereby saving valuable time and resources. This process not only helps in enhancing productivity but also ensures that employees can efficiently address inquiries, leading to improved operational efficiency and better organisational decision-making. Most importantly, LLMs empower the customer support team to enhance its efficiency in answering queries and providing assistance, thereby improving customer relationships and retention rates by reducing churn and enhancing overall satisfaction with the support services provided. Overall, integrating LLMs into organisational workflows provides a multitude of benefits to employees and customers. 
